Search for Anomalous Production of Events with a High Energy Lepton and Photon at the Tevatron

We present results of a search for for the anomalous production of events containing a high-transverse momentum charged lepton (electron or muon) and photon, accompanied by missing transverse energy (MET), and/or additional leptons and photons, and jets (X). We use the same kinematic selection criteria as in a previous CDF search, but with a substantially larger data set, 305pb-1, a ppbar collision energy of 1.96 TeV, and the upgraded CDF II detector. We find 42 Lepton + Photon + MET events versus a standard model expectation of 37.3 +- 5.4 events. The level of excess observed in Run I, 16 events with an expectation of 7.6 +- 0.7 events (corresponding to a 2.7 sigma effect), is not supported by the new data. In the signature of Multi-Lepton + Photon we observe 31 events versus an expectation of 23.0 +- 2.7 events. In this sample we find no events with an extra photon or MET and so find no events like the one 'two electrons + two photons + MET' ('eeggmet') event observed in Run I.

==> en_disser_events.tex <==
\section{Some comments on the events}

For the $\lgmet$ Lepton $\Pt$ distribution we have two events with a
high-$\Pt$ Lepton in the same bin. One of the events come from the
muon channel, one from the electron channel:

\subsection{$\mugmet$ and $\egmet$ Candidate Events}
\begin{small}

\vskip-0.1in
\begin{table}[!h]
\begin{center}
\input{muon/tables/r166008_e3466824.table}
\caption{$\mugmet$ Candidate Event}
\end{center}
\end{table}

\begin{table}[!h]
\begin{center}
\input{electron/tables/r184778_e6449604.table}
\caption{$\egmet$ Candidate Event}
\end{center}
\end{table}

\end{small}


==> local_tables/lepton_photon_summaryt <==
\newcommand{\noflg}{574}
\newcommand{\noflgpb}{1.88}
\newcommand{\dnoflgpb}{0.079}
\newcommand{\noflgdphi}{422}
\newcommand{\noflgdphipb}{1.38}
\newcommand{\dnoflgdphipb}{0.067}
\newcommand{\noflgzlike}{218}
\newcommand{\noflgzlikepb}{0.71}
\newcommand{\dnoflgzlikepb}{0.048}
\newcommand{\noflgzunlike}{79}
\newcommand{\noflgzunlikepb}{0.26}
\newcommand{\dnoflgzunlikepb}{0.029}
\newcommand{\noflgtwobody}{204}
\newcommand{\noflgtwobodypb}{0.67}
\newcommand{\dnoflgtwobodypb}{0.047}
\newcommand{\noflgzlikeruni}{172}
\newcommand{\noflgzlikerunipb}{0.56}
\newcommand{\dnoflgzlikerunipb}{0.043}
\newcommand{\noflgtwobodyruni}{250}
\newcommand{\noflgtwobodyrunipb}{0.82}
\newcommand{\dnoflgtwobodyrunipb}{0.052}
\newcommand{\noflgallother}{152}
\newcommand{\noflgallotherpb}{0.50}
\newcommand{\dnoflgallotherpb}{0.040}
\newcommand{\noflglgmet}{42}
\newcommand{\noflglgmetpb}{0.14}
\newcommand{\dnoflglgmetpb}{0.021}
\newcommand{\noflgmultil}{31}
\newcommand{\noflgmultilpb}{0.10}
\newcommand{\dnoflgmultilpb}{0.018}
\newcommand{\noflgmultig}{0}
\newcommand{\noflgmultigpb}{0}
\newcommand{\dnoflgmultigpb}{0}
\newcommand{\noflgmultilgmet}{0}
\newcommand{\noflgmultilgmetpb}{0}
\newcommand{\dnoflgmultilgmetpb}{0}


==> local_tables/ru_gelectron_sample.tex <==
%\documentstyle[11pt]{report}
%\begin{document}
\begin{figure*}[h]
\thicklines
\begin{center}
\framebox(155,70)[s]{
{
\begin{minipage}{150pt}
\begin{center}
$\eg$ образец \\
1 электрон и 1 фотон \\
$\Etelectron>25\GeV$, $\Etgamma>25\GeV$ \\
%$E_T\gt 25$ GeV \\
{\bf\nofeg} событий
\end{center}
\end{minipage}
}
}
\put(-10,0){\vector(0,-1){60}}
\put(-140,0){\vector(0,-1){60}}
\vspace{-1pt}

\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 электрон \\
Ровно 1 фотон \\
$\Delta\phi_{\eg}\gt 150$ \\
$\met\lt 25$ \\
{\bf\nofegdphi} событий
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){32}}
\put(-130,0){\vector(0,-1){135}}
\makebox(30,60)[l]{}
\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Несколько объектов \\
(Все остальные $\eg$) \\
{\bf\nofegallother} событий
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){135}}
\put(-130,0){\vector(0,-1){135}}
\put(-75,0){\vector(0,-1){32}}
\end{center}

\vspace{-118pt}

%Landscape
%\makebox(243,60)[l]{}
%Portrait
\makebox(110,60)[l]{}
\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
$\Z$-подобные $\eg$ \\
81 Gev $\lt M_{\eg}\lt$ 101 Gev\\
(Оценка фона) \\
{\bf\nofegzlike} событий
\end{center}
\end{minipage}
}
}
\makebox(20,60)[l]{}
\framebox(100,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 электрон \\
Ровно 1 фотон \\
$\Delta\phi_{\eg}\lt 150$ \\
$\met\lt 25$ GeV \\
{\bf\nofegzunlike} событий
\end{center}
\end{minipage}
}
}

\begin{center}
\framebox(115,70)[0,0]{
{
\begin{minipage}{115pt}
\begin{center}
Два объекта \\
{\bf \nofegtwobody} событий
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События типа $\egmet$\\
$\met\gt 25$ GeV \\
{\bf \nofeglgmet} событий
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События типа \\
$\egg$ и $\eeg$ \\
{\bf\nofegmultig} и {\bf\nofegmultil} событий, соответственно
\end{center}
\end{minipage}
}
}
\end{center}
%\end{document}\caption{электрон Control Sample}
\caption
[Электрон-фотонный образец: категории инклюзивных $\egX$ событий]
{Электрон-фотонный образец: категории инклюзивных $\egX$ событий.}
\label{flowchart_electron.figure}
\end{figure*}


==> local_tables/ru_glepton_sample.tex <==
%\documentstyle[11pt]{report}
%\begin{document}
\begin{figure*}[h]
\thicklines
\begin{center}
\framebox(155,70)[s]{
{
\begin{minipage}{150pt}
\begin{center}
$\lg$ образец \\
1 лептон и 1 фотон \\
$\Etlepton>25\GeV$, $\Etgamma>25\GeV$ \\
{\bf\noflg} событий
\end{center}
\end{minipage}
}
}
\put(-10,0){\vector(0,-1){60}}
\put(-140,0){\vector(0,-1){60}}
\vspace{-1pt}

\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 лептон \\
Ровно 1 фотон \\
$\Delta\phi_{l\gamma}\gt 150$ \\
$\met\lt 25$ \\
{\bf\noflgdphi} событий
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){32}}
\put(-130,0){\vector(0,-1){135}}
\makebox(30,60)[l]{}
\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Несколько объектов \\
(Все остальные $\lg$) \\
{\bf\noflgallother} событий%($ll\gamma$, $l\gamma\met$)
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){135}}
\put(-130,0){\vector(0,-1){135}}
\put(-75,0){\vector(0,-1){32}}
\end{center}

\vspace{-118pt}




\makebox(110,60)[l]{}
\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
$\Z$-подобные $\lg$ \\
%86 Gev$~<~M_{e\gamma}~<~$96 Gev\\
81 Gev $\lt M_{\ell\gamma}\lt$ 101 Gev\\
(Оценка фона) \\
{\bf\noflgzlike} событий
\end{center}
\end{minipage}
}
}
\makebox(20,60)[l]{}
\framebox(100,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 лептон \\
Ровно 1 фотон \\
$\Delta\phi_{l\gamma}\lt 150$ \\
$\met\lt 25$ GeV \\
{\bf\noflgzunlike} событий
\end{center}
\end{minipage}
}
}

\begin{center}
\framebox(115,70)[0,0]{
{
\begin{minipage}{115pt}
\begin{center}
Два объекта \\
{\bf\noflgtwobody} событий
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События типа $\lgmet$\\
$\met\gt 25$ GeV \\
{\bf\noflglgmet} событий%($l\gamma\met$)
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События типа \\
$\lgg$ и $\llg$ \\
{\bf\noflgmultig} и {\bf\noflgmultil} событий, соответственно
\end{center}
\end{minipage}
}
}
%\end{picture}
\end{center}
%\end{document}\caption{Muon Control Sample}
\caption
[Лептон-фотонный образец: категории инклюзивных $\lgX$ событий]
{Лептон-фотонный образец: категории инклюзивных $\lgX$ событий.}
\label{flowchart_lepton.figure}
\end{figure*}


==> local_tables/ru_glepton_sample_auto.tex <==
%\documentstyle[11pt]{report}
%\begin{document}
\begin{figure*}[h]
\thicklines
\begin{center}
\framebox(155,70)[s]{
{
\begin{minipage}{150pt}
\begin{center}
$\lg$ образец \\
1 лептон и 1 фотон \\
$\Etlepton>25\GeV$, $\Etgamma>25\GeV$ \\
{\bf\noflg} событий
\end{center}
\end{minipage}
}
}
\put(-10,0){\vector(0,-1){15}}
\put(-140,0){\vector(0,-1){15}}
\vspace{-1pt}

\framebox(150,80)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 лептон \\
Ровно 1 фотон \\
$\Delta\phi_{l\gamma}\gt 150$ \\
$\met\lt 25$ \\
{\bf\noflgdphi} событий
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){32}}
\put(-130,0){\vector(0,-1){135}}
\makebox(30,60)[l]{}
\framebox(150,80)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Несколько объектов \\
(Все остальные $\lg$) \\
{\bf\noflgallother} событий%($ll\gamma$, $l\gamma\met$)
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){125}}
\put(-130,0){\vector(0,-1){125}}
\put(-75,0){\vector(0,-1){32}}
\end{center}

\vspace{-118pt}




\makebox(110,60)[l]{}
\framebox(150,80)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
$\Z$-подобные $\lg$ \\
%86 Gev$~<~M_{e\gamma}~<~$96 Gev\\
81 Gev $\lt M_{\ell\gamma}\lt$ 101 Gev\\
(Оценка фона) \\
{\bf\noflgzlike} событий
\end{center}
\end{minipage}
}
}
\makebox(20,60)[l]{}
\framebox(90,80)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 лептон \\
Ровно 1 фотон \\
$\Delta\phi_{l\gamma}\lt 150$ \\
$\met\lt 25$ GeV \\
{\bf\noflgzunlike} событий
\end{center}
\end{minipage}
}
}

\begin{center}
\framebox(115,70)[0,0]{
{
\begin{minipage}{115pt}
\begin{center}
Два объекта \\
{\bf\noflgtwobody} событий
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События вида $\lgmet$\\
$\met\gt 25$ GeV \\
{\bf\noflglgmet} событий%($l\gamma\met$)
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События вида \\
$\lgg$ и $\llg$ \\
{\bf\noflgmultig} и {\bf\noflgmultil} событий, соответственно
\end{center}
\end{minipage}
}
}
%\end{picture}
\end{center}
%\end{document}\caption{Muon Control Sample}
\caption
[Лептон-фотонный образец: категории инклюзивных $\lg$ событий]
{Лептон-фотонный образец: категории инклюзивных $\lg$ событий.}
\label{flowchart_lepton.figure}
\end{figure*}


==> local_tables/ru_gmuon_sample.tex <==
%\documentstyle[11pt]{report}
%\begin{document}
\begin{figure*}[h]
\thicklines
\begin{center}
\framebox(155,70)[s]{
{
\begin{minipage}{150pt}
\begin{center}
$\mug$ образец \\
1 мюон и 1 фотон \\
$\Ptmuon>25\GeV$, $\Etgamma>25\GeV$ \\
{\bf\nofmug} событий
\end{center}
\end{minipage}
}
}
\put(-10,0){\vector(0,-1){60}}
\put(-140,0){\vector(0,-1){60}}
\vspace{-1pt}

\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 мюон \\
Ровно 1 фотон \\
$\Delta\phi_{\mug}\gt 150$ \\
$\met\lt 25$ \\
{\bf\nofmugdphi} событий
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){32}}
\put(-130,0){\vector(0,-1){135}}
\makebox(30,60)[l]{}
\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Несколько объектов \\
(Все остальные $\mug$) \\
{\bf\nofmugallother} событий
\end{center}
\end{minipage}
}
}
\put(-20,0){\vector(0,-1){135}}
\put(-130,0){\vector(0,-1){135}}
\put(-75,0){\vector(0,-1){32}}
\end{center}

\vspace{-118pt}

%Landscape
%\makebox(243,60)[l]{}
%Portrait
\makebox(110,60)[l]{}
\framebox(150,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
$\Z$-подобные $\mug$ \\
81 Gev $\lt M_{\mug}\lt$ 101 Gev\\
(Background Calibration) \\
{\bf\nofmugzlike} событий
\end{center}
\end{minipage}
}
}
\makebox(20,60)[l]{}
\framebox(100,90)[0,0]{
{
\begin{minipage}{150pt}
\begin{center}
Ровно 1 мюон \\
Ровно 1 фотон \\
$\Delta\phi_{\mug}\lt 150$ \\
$\met\lt 25$ GeV \\
{\bf\nofmugzunlike} событий
\end{center}
\end{minipage}
}
}

\begin{center}
\framebox(115,70)[0,0]{
{
\begin{minipage}{115pt}
\begin{center}
Два объекта \\
{\bf \nofmugtwobody} событий
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События типа $\mugmet$\\
$\met\gt 25$ GeV \\
{\bf \nofmuglgmet} событий
\end{center}
\end{minipage}
}
}
\framebox(115,70)[0,0]{
{
\color{red}
\begin{minipage}{115pt}
\begin{center}
События типа \\
$\mugg$ и $\mumug$ \\
{\bf\nofmugmultig} и {\bf\nofmugmultil} событий, соответственно
\end{center}
\end{minipage}
}
}
\end{center}
%\end{document}\caption{мюон Control Sample}
\caption
[Мюон-фотонный образец: категории инклюзивных $\mugX$ событий]
{Мюон-фотонный образец: категории инклюзивных $\mugX$ событий.}
\label{flowchart_muon.figure}
\end{figure*}

